Scalable Normalizing Flows Enable Boltzmann Generators for Macromolecules

The Boltzmann distribution of a protein provides a roadmap to all of its functional states. Normalizing flows are a promising tool for modeling this distribution, but current methods are intractable for typical pharmacological targets; they become computationally intractable due to the size of the system, heterogeneity of intra-molecular potential energy, and long-range interactions. To remedy these issues, we present a novel flow architecture that utilizes split channels and gated attention to efficiently learn the conformational distribution of proteins defined by internal coordinates. We show that by utilizing a 2-Wasserstein loss, one can smooth the transition from maximum likelihood training to energy-based training, enabling the training of Boltzmann Generators for macromolecules. We evaluate our model and training strategy on villin headpiece HP35(nle-nle), a 35-residue subdomain, and protein G, a 56-residue protein. We demonstrate that standard architectures and training strategies, such as maximum likelihood alone, fail while our novel architecture and multi-stage training strategy are able to model the conformational distributions of protein G and HP35.

==> sections/related_works.tex <==
\section{Related Works}

% \subsection{Boltzmann Generators}
% Bolzmann generators \citep{noe2019bg} are normalizing flows that approximate Boltzmann distributions. \cite{noe2019bg} utilized the fact that normalizing flows are tractable density models and introduced a notion of training by energy via reverse KL-divergence minimization. Recently, there has been a growing interest in Boltzmann generators. \cite{dibak2021tempbg} proposed temperature steerable flows that generalized to families of ensembles across multiple temperatures, thereby increasing the range of thermodynamic states accessible for sampling. Unfortunately, this model tends to undersample significant local minimas for systems as small as alanine dipeptide. The authors believed that this was due to the limited expressivity of the flow model. \cite{wu2020stochastic} proposed stochastic normalizing flows, which combine flows with MCMC methods by introducing sampling layers between flow layers to improve model expressivity. Unfortunately, this method is computationally expensive as it involves many more target evaluations. In addition, stochastic normalizing flows tend to miss modes \citep{midgley2022fab}. \cite{kohler2021smoothnf} introduced smooth normalizing flows, which are $C^\infty$-smooth, thus making them more physically amenable. They also introduce force-matching as an added loss term. While they have impressive results and modal coverage for alanine dipeptide, they utilize a root-finding algorithm to approximate the inverse for their smooth flows, which becomes computationally prohibitive for higher-dimensional systems. 

% This work has focused on normalizing flows. However, diffusion models have also shown great promise as an alternative generative model for learning Boltzmann generators. \cite{jing2022torsionaldiff} train a diffusion model to learn the Boltzmann distribution over the torsion angles of multiple drug-like molecules, while using cheminformatics methods for the bond lengths and angles. They perform energy-based training (similar in spirit to the reverse KL divergence in flow model training) via estimation of a score matching loss using samples generated by the model. However, this method does not scale well to larger molecules and inherits the same problem of unstable training at initialization. 

% \subsection{Loss functions}
% \cite{wirnsberger2022nf} trained a flow model without MD samples by minimizing the KL divergence to approximate the Boltzmann distribution of atomic solids with up to 512 atoms. However, the KL-divergence suffers from mode-seeking behavior, which severely impairs training for multimodal target distributions. While the forward KL-divergence, i.e. maximum likelihood, is mass covering, the Monte Carlo approximations of such an objective have a very high variance in loss. To circumvent this, \cite{midgley2022fab} trains a flow to approximate a target $p$ by minimizing the alpha-divergence with $\alpha = 2$, which is estimated with annealed importance sampling (AIS) using the flow $q$ as the base distribution and $p^2/q$ as target. This method is notable in that it does not require any MD samples but still achieves impressive results for alanine dipeptide. Nonetheless, the AIS component is computationally expensive and scales poorly for larger systems. 

% \subsection{Coarse-graining}

% Several works have attempted to scale flow-based Boltzmann generators to larger systems. \cite{mahmoud2022coarse} trained a flow model on coarse-grained protein representations which they then mapped back to full-atom representations using a language model. On a similar note, \cite{kohler2022flowmatching} trained a normalizing flow to represent the probability density for coarse-grained (CG) MD samples in order to learn the parameters of a CG model. Unfortunately, coarse-grain approaches tend to lose significant information compared to full-atom resolution for downstream applications. Importantly, both works note that using internal-coordinate representations do not scale well as small changes in torsion angles can lead to large global distortions. Our results indicate that this is not necessarily true, as we use a reduced internal-coordinate representation. 

% \subsection{Normalizing flow architectures}
% Our flow model, while novel, shares some similarities to previous works. DenseFlow \cite{grcic2021densely} fuses a densely connected convolutional block with Nystr\"{o}m self-attention in modules with both cross-unit and intra-module couplings. This architecture is specifically designed for image data and utilizes a linear approximation for the self-attention mechanism. In contrast, we use gated attention and rotary positional embeddings in order to handle the sequential nature of proteins. In the protein domain, previous works also split the inputs into different channels \cite{noe2019bg,kohler2021smoothnf,kohler2022flowmatching}. However, they split the input dimensions into torsion, angle, and bond channels. In contrast, our model splits the input into separate backbone and sidechain channels to better capture the global distribution.
